A Theory of Lazy Imperative Timing

We present a theory of lazy imperative timing.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{J. Derrick, B. Dongol and S. Reeves (Eds.):\\ Refinement Workshop 2018 (REFINE'18).\\
EPTCS 282, 2018, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.282.1}{10.4204/EPTCS.282.1}}

